Divide-and-Rule: Self-Supervised Learning for Survival Analysis in Colorectal Cancer

With the long-term rapid increase in incidences of colorectal cancer (CRC), there is an urgent clinical need to improve risk stratification. The conventional pathology report is usually limited to only a few histopathological features. However, most of the tumor microenvironments used to describe patterns of aggressive tumor behavior are ignored. In this work, we aim to learn histopathological patterns within cancerous tissue regions that can be used to improve prognostic stratification for colorectal cancer. To do so, we propose a self-supervised learning method that jointly learns a representation of tissue regions as well as a metric of the clustering to obtain their underlying patterns. These histopathological patterns are then used to represent the interaction between complex tissues and predict clinical outcomes directly. We furthermore show that the proposed approach can benefit from linear predictors to avoid overfitting in patient outcomes predictions. To this end, we introduce a new well-characterized clinicopathological dataset, including a retrospective collective of 374 patients, with their survival time and treatment information. Histomorphological clusters obtained by our method are evaluated by training survival models. The experimental results demonstrate statistically significant patient stratification, and our approach outperformed the state-of-the-art deep clustering methods.

==> MICCAI 2020 - Divide and Rule/files/abstract.tex <==
\begin{abstract}
With the long-term rapid increase in incidences of colorectal cancer (CRC), there is an urgent clinical need to improve risk stratification. The conventional pathology report is usually limited to only a few histopathological features. However, most of the tumor microenvironments used to describe patterns of aggressive tumor behavior are ignored. In this work, we aim to learn histopathological patterns within cancerous tissue regions that can be used to improve prognostic stratification for colorectal cancer. To do so, we propose a self-supervised learning method that jointly learns a representation of tissue regions as well as a metric of the clustering to obtain their underlying patterns. These histopathological patterns are then used to represent the interaction between complex tissues and predict clinical outcomes directly. We furthermore show that the proposed approach can benefit from linear predictors to avoid overfitting in patient outcomes predictions. To this end, we introduce a new well-characterized clinicopathological dataset, including a retrospective collective of 374 patients, with their survival time and treatment information. Histomorphological clusters obtained by our method are evaluated by training survival models. The experimental results demonstrate statistically significant patient stratification, and our approach outperformed the state-of-the-art deep clustering methods. %  and proposed dataset 

\keywords{Self-supervised learning \and Histology \and Survival analysis \and Colorectal cancer.}
\end{abstract}

==> MICCAI 2020 - Divide and Rule/files/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We have proposed a self-supervised learning method that offers a new approach to learn histopathological patterns within cancerous tissue regions. Our model presents a novel way to model the interactions between tumor-related image regions and tackles the inherent overfitting problem to predict patient outcome. Our method surpasses all previous baseline methods and histopathological features and achieves state-of-the-art results, i.e., in C-Index without any data-specific annotation. Ablation studies also show the importance of different components of our method and the relevance of combining them. We envision the broad application of our approach for clinical prognostic stratification improvement.

%\tikz[overlay,remember picture]
%    \draw (current page.west) -- (current page.east);



==> MICCAI 2020 - Divide and Rule/files/introduction.tex <==
\section{Introduction}
Colorectal cancer is the third leading cause of cancer-related mortality worldwide. Five-year survival rates are low, at 60$\%$. Although standard histopathological of cancer reporting based on features such as staging and grading identifies patients with a potentially worse outcome to therapy, there is still an urgent need to improve risk stratification. Pathologists typically limit their reporting of colorectal cancers to approximately ten features, which they describe as single elements in their report (e.g., depth of invasion, pT; lymph node metastasis, etc.). However, the histopathological (H\&E) slide is a “snapshot” of all occurring tumor-related processes, and their interactions may hold a wealth of information that can be extracted to help refine prognostication. These slides can then be digitized and used as input for computational algorithms to help support pathologists in their decision-making. The distribution of tissue types within the slide, the proximity of cell types or tissue components, and their spatial arrangement throughout the tissue can identify new patterns not previously detectable to the human eye alone.

Few studies have performed unsupervised clustering of whole slide images (WSIs) based on patch descriptors. They have been used to address the problem of image segmentation \cite{moriya2018unsupervised} or latent space clustering \cite{dercksen2019dealing,fouad2017unsupervised}. Among DL-based survival models, a recent study \cite{kather2019predicting} used a supervised CNN for end-to-end classification of tissues to predict the survival of patients with colorectal cancer. 
\begin{comment}
In \cite{nirschl2018deep}, CNN based model was used to predict cardiac outcome from endomyocardial biopsy. 
\end{comment}
Similar to our approach, several recent works have proposed unsupervised methods \cite{muhammad2019unsupervised,zhu2017wsisa,li2018graph} for slide-level survival analysis. In \cite{zhu2017wsisa}, one of the first unsupervised approaches, DeepConvSurv has been proposed for survival prediction based on WSIs. More recently, DeepGraphSurv \cite{li2018graph} has been presented to learn global topological representations of WSI via graphs. However, they heavily relied on noisy compressed features from a pre-trained VGG network. Recently, self-supervised representation learning methods \cite{he2020momentum,zhuang2019local,chen2020simple} have been proposed to utilize the pretext task for extracting generalizable features from the unlabeled data itself. Therefore, the dataset does not need to be manually labeled by qualified experts to solve the pretext task. 

\subsubsection{Contributions.} In this work, we propose a new approach to learn histopathological patterns through self-supervised learning within each WSI. Besides, we present a novel way to model the interaction between tumor-related image regions for survival analysis and tackle the inherent overfitting problem on tiny patient sets. To this end, we take advantage of a well-characterized, retrospective collective of 374 patients with clinicopathological data, including survival time and treatment information. H\&E slides were reviewed, and at least one tumor slide per patient was digitized. To accelerate research we have made our code and trained models publicly available on GitHub.\footnote{https://github.com/christianabbet/DnR}

 

==> MICCAI 2020 - Divide and Rule/files/method.tex <==
\section{Method}
\label{sec:method}
We first introduce our self-supervised image representation (Sec. \ref{subsec:SelfSupervised}) for the cancerous tissue area identified by our region of interest (RoI) detection scheme (Sec. \ref{subsec:RoIDetection}). Then, we propose our deep clustering scheme and baseline algorithms in Sec. \ref{subsec:ProposedApproach} and Sec. \ref{subsec:Algorithm Baselines}, respectively. The clustering approach's usefulness is assessed by conducting survival analysis (Sec. \ref{subsec:SurvivalAnalysis}) to measure if the learned clusters can contribute to disease prognostication. Finally, we discuss our implementation setup and experimental results in Sec. \ref{sec:experimentalResults}.

\subsection{RoI Detection}
\label{subsec:RoIDetection}
Our objective is to learn discriminative patterns of unhealthy tissues of patients. However, WSI does not include information about the cancerous regions or the location of the tumor itself. Therefore, we seek a transfer learning approach for the classification of histologic components of WSIs. To do so, we choose to use the dataset presented in \cite{kather19dataset} to train a classifier to discriminate relevant areas. The dataset is composed of 100K examples of tissue from CRC separated into nine different classes. For our task, we choose to retain three classes: lymphocytes (LYM), cancer-associated stroma (STR), and colorectal adenocarcinoma epithelium (TUM) that show the discriminative evidence for the class-of-interest and have been approved by the pathologist. Note that the presence of a large number of lymphocytes around the tumor is an indication of the immune reaction and, therefore, possibly linked to a higher survival score. We first train our classifier with the ResNet-18 backbone \cite{he16}. Then we use the stain normalization approach proposed in \cite{macenko09stain} to match the color space of the target domain and prevent the degradation of the classifier on transferred images. An example of RoI estimation is presented in Fig. \ref{fig:model_pipeline}. Such a technique allows us to discard a large part of the healthy tissue regions.


%The model backbone is initialized with pretrained weights, and classification layers are trained from scratch. It achieves similar classification performances as mentioned in \cite{kather19}. When applying the model on our data, we use the stain normalization approach proposed in \cite{macenko09stain} to match the color space of the target domain. 
\begin{comment}
\begin{figure*}[ht]
\centering
\includegraphics[width=\linewidth]{medias/seg_003c.pdf}
\caption{Source image crop (left). The foreground mask estimated using color thresholds and morphology (center). Samples located outside the mask are discarded during embedding space training. Classifier trained on \cite{kather19dataset} is used to assign patches to 9 classes (right). Only LYM, STR, TUM are kept to generate an estimation of the region of interest. }
\label{fig:mask_roi}
\end{figure*}
\end{comment}

\subsection{Self-Supervised Representation Learning}
\label{subsec:SelfSupervised}
In this paper, we propose a self-supervised transfer colorization scheme to learn a more meaningful feature representation of the tissues and reduce the requirement for intensive tissue labeling. Unsupervised learning methods such as autoencoder trained by minimizing reconstruction error tend to ignore the underlying structure of the image as the model usually learns the distribution of the color space. To avoid this issue, we use colorization learning as a proxy task. As the input image, we convert the original unlabeled image through mapping function $\zeta(x)$ to a two-channel image (hematoxylin and eosin) that describes the nuclei and amount of extracellular material, respectively. To sidestep the memory bottleneck, we represent the WSI as a set of adjacent/overlapping tiles (image patches) $\left \{x_i \in \mathcal{X} \right \}^N_{i=1}$. 

\begin{comment}
\begin{figure*}[ht]
\centering
\includegraphics[width=\linewidth]{medias/model.pdf}
\caption{Proposed architecture. The sample input, $x_i$, is converted to HE through $\zeta(x_i)$ and fed to the autoencoder. $\mathcal{L}_{\text{MSE}}$ is the reconstruction loss and $\mathcal{L}_{\text{Z}}$ the additional loss applied on the embedding space to constrain feature representation learning.}
\label{fig:model_cae}
\end{figure*}
\end{comment}



\begin{comment}
We train a convolutional auto encoders (CAE) to measure per-pixel difference between reconstructed image(s) and input image(s) using MSE loss:

\begin{equation}
    \mathcal{L}_{\text{MSE}}= \min\limits_{\phi, \psi} \left \| x- \psi \circ \phi \left ( x \right )\right \|_{2}^{2}
    \label{eq:autoencoder}
\end{equation}
%
\end{comment}

We define a function $\zeta : \mathcal{X} \rightarrow \mathcal{X}^{HE}$ that converts the input images to their HE equivalent \cite{macenko09stain,vahadane16stain}. Then, we train a convolutional autoencoder (CAE) to measure the per-pixel difference between transformed image(s) and input image(s) using MSE loss:

\begin{equation}
    \min\limits_{\phi, \psi} \mathcal{L}_{\text{MSE}}= \min\limits_{\phi, \psi} \left \| x- \psi \circ \phi \circ \zeta \left ( x \right )\right \|_{2}^{2}
    \label{eq:autoencoder_selfsup}.
\end{equation}

%A similar approach was proposed in \cite{zhang17splitbrain} where the encoder, $\phi$ is replaced by a set of encoders, $\{\phi_i\}_{i=1}^F$, to process each channel individually. In histology, the relation between H and E stain is crucial to determinate the properties of tissue. 

The encoder $\phi: \mathcal{X}^{HE} \rightarrow \mathcal{Z}$ is a convolutional neural network that maps an input image to its latent representation $\mathcal{Z}$. The decoder $\psi: \mathcal{Z} \rightarrow \mathcal{X}$ is an up-sampling convolutional neural network that reconstructs the input image given a latent space representation. As a result, we use a single input branch to take into account the tissue's structural aspect.

% no space, and achieve a proper reconstruction
%The decoder is created by alternating convolutional layers and bilinear up-sampling until reaching the desired output dimension. The architecture of the decoder was selected to have a minimal number of parameters. This approach allows us to ensure that the encoder will generates a meaningful latent space as the decoder is not complex enough to achieve perfect samples reconstructions. 


\subsection{Proposed Divide-and-Rule Approach}
\label{subsec:ProposedApproach}
The principle behind our self-supervised learning approach is to represent image patches based on their spatial proximity in the feature space, meaning any two adjacent image patches (positive pairs) are more likely to be close to each other in the feature space $\mathcal{Z}$ than two distant patches (negative pairs). Such characteristics are met for overlapping patches as they share similar histomorphological patterns. We let $\mathcal{S}_i$ denote the set of patches that overlap with patch $i$ spatially. Besides, we can assume that image patches in which their relative distances are smaller than a proximity threshold in the feature space should share common patterns. We define $\mathcal{N}_i$ as the set of top-$k$ patches that achieve the lowest cosine distance to the embedding $z_i$ of the image patch $i$. 
%\textcolor{red}{Todo, maybe say two way of being similar S and N.}

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{medias/sketch_pipeline_full.pdf}
    \caption{\textbf{The pipeline of the proposed approach.} Estimation of the region of interest (a),  learning of the embedding space (b-c), fitting of the cluster, assignment of all patient patches, and survival analysis (d-f).}
    \label{fig:model_pipeline}
\end{figure}

Firstly, we initialize the network parameters using the self-supervised reconstruction loss in Eq. \ref{eq:autoencoder_selfsup}. Then, for each patch embedding $i$, we label its overlapping set of patches $\mathcal{S}_i$ as similar patches (positive pairs). Otherwise, we consider any distant patches as a negative pair, whose embeddings should be scattered. Motivated by \cite{wu2018unsupervised}, we use a variant of the cross-entropy to compute the instance loss (Eq.~\ref{eq:divide}):
%It is important to avoid adding additional constraints while initializing the network as the distribution of the latent space is not yet stable and would therefore altered the quality of the convergence. \cite{wu2018unsupervised}


\begin{comment}
\begin{equation}
    p\left( j \mid i \right) = \frac{\exp{(z_{j}^T z_{i}/\tau )}}{\sum_{k=1}^N \exp{(z_{k}^T z_{i}/\tau )}}
    \label{eq:p_an}
\end{equation}
\end{comment}

\begin{equation}
    %\min\limits_{\phi} \mathcal{L}_{\text{Divide}} = -
    \mathcal{L}_{\text{Divide}}= -
    \sum_{i \in \mathcal{B}_{\text{inst}}} \log{(\sum_{j \in S_i} p\left( j \mid i \right))}\mathrm{,}\quad  p\left( j \mid i \right) = \frac{\exp{(z_{j}^{\top} z_{i}/\tau )}}{\sum_{k=1}^N \exp{(z_{k}^{\top} z_{i}/\tau )}}.
    \label{eq:divide}
\end{equation}

where $\tau \in \left ] 0,1 \right ]$ is the temperature parameter and $\mathcal{B}_{\text{inst}}$ denotes the set of samples in the mini-batch.  

Secondly, we jointly optimize the training of network with reconstruction loss and a Rule loss $\mathcal{L}_{\text{Rule}}$ that takes into account the similarity of different images in the feature space (Eq. \ref{eq:rule}). We gradually expand the vicinity of each sample to select its neighbor samples. If samples have high relative entropy, they are dissimilar and should be considered as individual classes, $z \in \mathcal{B}_{\text{inst}}$. On the contrary, if samples have low relative entropy with their neighbors, they should be tied together, $z \in \mathcal{Z} \backslash \mathcal{B}_{\text{inst}}$. In practice, the entropy acts as a threshold to decide a boundary between close and distant samples and is gradually increased during training such that we go from easy samples (low entropy) to hard ones (high entropy). Finally, the proposed training loss, $\mathcal{L}_{\text{DnR}}$, joins the above losses with a weighting term $\lambda$ (see Eq. \ref{eq:an_dnr}):

\begin{equation}
    %\min\limits_{\phi} \mathcal{L}_{\text{Rule}} = \sum_{i \in \mathcal{Z}\backslash\mathcal{B}_{\text{inst}}} \log{( \sum_{j \in \mathcal{S}_i \cup \mathcal{N}_i} p\left( j \mid i \right))}
    \mathcal{L}_{\text{Rule}} = - \sum_{i \in \mathcal{Z}\backslash\mathcal{B}_{\text{inst}}} \log{( \sum_{j \in \mathcal{S}_i \cup \mathcal{N}_i} p\left( j \mid i \right))}.
    \label{eq:rule}
\end{equation}

\begin{equation}
    \min\limits_{\phi, \psi} \mathcal{L}_{\text{DnR}} = \min\limits_{\phi, \psi} \mathcal{L}_{\text{MSE}} + \lambda \min\limits_{\phi} [ \mathcal{L}_{\text{Divide}} + \mathcal{L}_{\text{Rule}}].
    \label{eq:an_dnr}
\end{equation}


\subsubsection{Dictionary Learning.} 
Measuring similarities between samples requires the computation of features in the entire dataset for each iteration. The complexity grows as a function of the number of samples in the dataset. To avoid this, we use a memory bank, where we keep track and update the dictionary elements as in \cite{zhuang2019local,wu2018unsupervised}.

%\cite{wu2018unsupervised,jiabo19an}.
% Measuring similarities between samples requires the computation of features in the entire dataset. To avoid this, we use a memory bank, where we update the dictionary elements.

%For each sample optimization, the model needs to estimate its feature similarity with respect to its neighbors which requires the computation of features in the entire dataset. To avoid this, we use a memory bank, where we update the dictionary elements.

\begin{comment} %We will add algorithm if we have enough space
\begin{algorithm}[htb]
\SetAlgoLined
\DontPrintSemicolon
\KwData{Training set of image patches $\{x_i \in \mathcal{X} \}^N_{i=1} $.}
\KwResult{Output cluster assignation $p \left( k \mid i \right)$. }
\textbf{Pre-Training:}\;
\nl\For{$t$ in $\{1, \ldots, N_{\text{Pre-train}}\}$}{
\nl     Train $\phi$ and $\psi$ using self-supervised image reconstruction loss, $\mathcal{L}_{MSE}$.\;
}
\textbf{Training:} \;
\nl \For{$r$ in $\{1, \ldots, N_{\text{Rounds}}\}$}{
\nl Increase entropy threshold and update the sets $\mathcal{B}_{\text{inst}}$ and $\mathcal{Z} \backslash \mathcal{B}_{\text{inst}}$ accordingly.\;
\nl \For{$t$ in $\{1, \ldots, N_{\text{Train}}\}$}{
\nl Mini-batch feed-forward through the network.\;
\nl Train $\phi$ and $\psi$ with objective loss computation $\mathcal{L}_{\text{DnR}}$.\;
\nl Dictionary feature refreshing.\;
}}

\nl Predict cluster assignment probability $p \left( k \mid i \right)$. \;
 \caption{Divide-and-Rule: Self-Supervised Learning Algorithm}
 \label{alg:unsupclust}
\end{algorithm}
\end{comment}


\subsection{Algorithm Baselines}
\label{subsec:Algorithm Baselines}
\subsubsection{Deep Clustering based on Spatial continuity (DCS).} As our first baseline, we leverage an inherent spatial continuity of WSIs. Spatially adjacent image patches (tiles) are typically more similar to each other than distant image patches in the slide and therefore should have similar feature representation $\mathcal{Z}$. Hence, we force the model to adopt such behavior by minimizing the distance between feature representations of a specific tile $z_i$ and its overlapping tiles $\mathcal{S}_i$. 
%$\sum_{j \in \mathcal{S}_i} \left \| z_i - z_j \right \|_{2}^{2}$. 
%The euclidean distance constrain can as well be replaced with different metrics such as cosine similarity or stochastic nearest neighbors \cite{hinton2015distilling}.
\begin{comment}
\begin{equation}
    \mathcal{L}_{\text{DCS}}=\min\limits_{\phi, \psi} \sum_{i=1}^N \mathcal{L}_{\text{MSE}}(x_i) + \lambda \sum_{j \in \text{sim}(z_i)} \left \| z_i - z_j \right \|_{2}^{2}
    \label{eq:l2}
\end{equation}
\end{comment}
%
\subsubsection{Deep Cluster Assignment (DCA).} The downside of the first baseline is that in some cases, two distant image patches may be visually similar, or there may exist some spatially close patches that are visually different. This introduces noise in the optimization process. To tackle this issue, we can impose cluster membership as in \cite{muhammad2019unsupervised}. 
%To do so, we initialize a set of $K$ clusters using K-Means algorithm. 

% with centers $U = \{\mu_k \subset \mathcal{Z}\}_{k=1}^K$, using K-Means algorithm. For each sample embedding, we compute its distance from the closest cluster center $\mu_k^{*}$, $\left \| z_i - \mu_k^{*} \right \|_{2}^{2} \text{, } \quad k = \arg\min\limits_{k} \left \| z_i - \mu_k \right \|_2$. 

%Note that cluster centers are re-estimated between each epoch and kept fixed during training and therefore, the technique cannot be considered as a joint learning approach.
\begin{comment}
\begin{equation}
    \mathcal{L}_{\text{DCA}}=\min\limits_{\phi, \psi} \sum_{i=1}^N \mathcal{L}_{\text{MSE}}(x_i) + \lambda  \left \| z_i - \mu_k^{*} \right \|_{2}^{2} \text{, } \quad k = \arg\min\limits_{k} \left \| z_i - \mu_k \right \|_2
    \label{eq:knn}
\end{equation}
\end{comment}
%
\subsubsection{Deep Embedded Clustering (DEC).} Unlike the second baseline, the objective of our last baseline is not only to determine the clusters but also to learn a meaningful representation of the tiles. Therefore, we consider to jointly learn deep feature representation ($\phi, \psi$) and image clusters $U$. The optimization is performed through the joint minimization of reconstruction loss and the KL divergence to gradually anneal cluster centers by fitting the model to an auxiliary distribution (see \cite{xie2016unsupervised} for details).



%we gradually anneal cluster centers by fitting the model to an auxiliary distribution $q$.
%More precisely, let $p \left( k \mid i \right)$ be the probability of assigning embedded sample $z_{i}$ to the cluster centroid $\mu _{k}$ as presented in \cite{xie2016unsupervised}. Instead of directly maximizing the cluster probability of the model $p$, we gradually anneal cluster centers by fitting the model to an auxiliary distribution $q$.
%We construct this target distribution, $q$, by first raising $p\left( k \mid i \right)$ to the second power to sharpen it, and then we normalize it by the frequency per cluster.
%The use of the variable $p$ is an example of soft clustering where a sample, $z_i$, can be tied to multiple cluster making the feature space representation more realistic.
\begin{comment}
\begin{equation}
    \mathcal{L}_{\text{DEC}} = \min\limits_{\phi, \psi, U} \mathcal{L}_{\text{MSE}}(x) + \lambda \ KL\left ( q\left |  \right |p \right ) 
    \label{eq:kl}
\end{equation}
\end{comment}

\begin{comment}%If we have enough space, we will add equations, otherwise we keep as it is.
\begin{equation}
    p \left( k \mid i \right) \propto\left ( 1+\left \| z_{i}-\mu _{k} \right \|^{2}_2 \right )^{-1} \quad\mathrm{and}\quad  q \left( k \mid i \right) \propto \frac{p \left( k \mid i \right)^{2}}{\sum_{i=1}^{N}p \left( k \mid i \right)}
    \label{eq:clusterassignment}
\end{equation}
\end{comment}

%In this work we present 4 novel approaches (Figure~\ref{fig:clustering}) to constrain features representation of histopathological images.

\input{files/method_survival}

==> MICCAI 2020 - Divide and Rule/files/method_survival.tex <==

\subsection{Survival Analysis}
\label{subsec:SurvivalAnalysis}

\subsubsection{Clustering and Assignment.} The learned embedding space is assumed to be composed of a limited number of homogeneous clusters. We fit spherical KMeans clustering (SPKM) \cite{skmc05zhon} to the learned latent space with $K$ clusters. As a result, every patch within a patient slide will be assigned to a cluster, $c_k = \argmin_{k \in \{0 \hdots K-1\}} \text{SPKM}(x_i, \mu_k)$.

%The representation of the patient should not depend on the number of the patches that are present in the slide.  (is it needed?)
Our objective is to model the interaction between tumor-related image regions (neighbor patches and clusters). To do so, we define a patient descriptor $h = [h^{C}, h^{T}] \in \mathbb{R}^{N \times (K+K^2)}$ as:

\begin{equation}
     h_{k}^{C} = p(s = k) \quad \text{and} \quad
    h_{j\rightarrow k}^{T} = p(s = k \mid N(s) = j),
    \label{eq:h_features}
\end{equation}

where $s$ is a patch, $h_{k}^{C}$ denotes the probability that a patch belongs to cluster $k$ and $h_{k}^{T}$ is the probability transition between a patch and its neighbors $N(s)$ (e.i. local interactions between clusters within the slide). 

\subsubsection{Survival.} Survival analysis is prone to overfitting as we usually rely on a small patient set and a large number of features. To counter this issue, we first apply forward variable selection \cite{muche2001applied} using log partial likelihood function with tied times \cite{coxtiedtimes77efron}, $\mathcal{L}_{\text{ll}}$, and likelihood-ratio (LR) test to identify the subset of relevant covariates:

\begin{equation}
    \text{LR} = -2[\mathcal{L}_{\text{ll}}( \beta^{\text{new}} \mid h^{\text{new}}) - \mathcal{L}_{\text{ll}}( \beta^{\text{prev}} \mid h^{\text{prev}})].
    \label{eq:forward}
\end{equation}

Here ${(h, \beta)}^{\text{prev}}$ and ${(h, \beta)}^{\text{new}}$ are the previous and new estimated set of covariates, respectively. To validate that the selected covariates do not overfit the patient data, we use leave-one-out cross-validation (LOOCV) on the dataset and predict linear estimators \cite{dai2019cross} as $\hat{\eta}_i = h_i \cdot \beta^{-i}$ and $\hat{\eta} = (\hat{\eta}_1, \hat{\eta}_2, \hdots \hat{\eta}_N)$ to compute C-Index \cite{multivariable96harrel}. Here, $\beta^{-i}$ is estimated on the whole patient set minus patient $i$. 




\begin{comment}
Survival analysis aims at finding a link between a set of variables and a time to event. More formally, given sets of time intervals, event observations, and features  $\{t_i \in \mathbb{R}^+, e_i \in \{0,1\}, h_i \in \mathbb{R}^D\}_{i=1}^N$ we aim at minimizing the partial likelihood:

\begin{equation}
    \mathcal{L}_{\text{ll}} = \min\limits_{\beta} \prod_{i=1}^N \left[ \frac{\theta_i}{\sum_{j \in R(t_i)} \theta_j} \right]^{e_i} \quad \text{and} \quad R(t_i) = \{j | t_j \leq t_i\},
    \label{eq:ph}
\end{equation}

where $\theta_i = \exp{(h_i^T\beta)}$ is the hazard ratio and $\beta$ the parameter weighting the contribution of each feature $h_i$. 


Survival analysis is prone to overfitting as we usually rely on a small patient set. To counter this issue, we propose to jointly benefit from linear predictors \cite{dai2019cross} and covariate stepwise selection \cite{muche2001applied}. We first apply forward variable selection with $\chi^2$ test:

\begin{equation}
    -2[\mathcal{L}_{\text{ll}}(\beta^{\text{new}}) - \mathcal{L}_{\text{ll}}(\beta^{\text{prev}})] \leq \chi^2(1)
    \label{eq:forward}
\end{equation}

where we $\beta^{\text{prev}}$ and $\beta^{\text{new}}$ are respectively the previous set of covariates and the set that contains the previous one plus the additional variable whose statistical influence to the model is being tested.


To validate that the selected set is not overfitting, we use linear predictor $\hat{\eta}_C$ on a set of covariates $C$, we compare its statistical 


To validate that the selected covariates are not overfitting the patient data, we use leave-one-out cross-validation (LOOCV) on the dataset and predict linear estimators as $\hat{\eta}^{cv}_i = h_i^T \beta^{-i}$ and $\hat{\eta}^{cv} = (\hat{\eta}^{cv}_1, \hat{\eta}^{cv}_2, \hdots \hat{\eta}^{cv}_N)$, where $\beta^{-i}$ is estimated on the whole patient set minus patient $i$. 

\end{comment}

==> MICCAI 2020 - Divide and Rule/files/results.tex <==
\section{Experimental Results}
\label{sec:experimentalResults}

\subsubsection{Dataset.}

We use a set of 660 in-house unlabeled WSIs of CRC stained with hematoxylin and eosin (H\&E). The slides are linked to a total of 374 unique patients diagnosed with adenocarcinoma. The dataset was filtered such that we exclude cases of mucinous adenocarcinoma in which their features are considered independent with respect to standard adenocarcinoma. A set of histopathological features (HFs) is associated with each patient entry (e.i. depth of invasion, pT, etc.). The survival time is defined as the period between resection of the tissue (operation) and the event occurrence (death of the patient). We denote $\mathcal{D}^{S}$ as the dataset that contains slides images and $\mathcal{D}^{S \cap HF}$ as the dataset that contains both information of the HFs and slides for each patient. Note that $|\mathcal{D}^{S \cap HF}| < |\mathcal{D}^{S}|$ as some patients have missing HFs and were excluded.

\subsubsection{Experimental Settings.}
We use ResNet-18 for the encoder where the input layer is updated to support 2 input channels. The latent space has dimensions $d=512$. The decoder is a succession of convolutional layers, ReLUs, and up-samplings (bicubic). The model was trained with the reconstruction loss $\mathcal{L}_{\text{MSE}}$ for 20 epochs with early stopping. We use Adam optimizer $\beta=(0.9, 0.999)$ and learning rate, $lr = 1\mathrm{e}{-3}$. Then, we add $\mathcal{L}_{\text{Divide}}$ for an additional 20 epochs with $\lambda = 1\mathrm{e}{-3}$ and $\tau=0.5$. Finally, we go through 3 additional rounds using $\mathcal{L}_{\text{Rule}}$ while raising the entropy threshold between each round. 

\begin{figure}[t!]
\centering
  \includegraphics[width=\linewidth]{medias/surv_km_hr.pdf}
    \caption{\textbf{Comparison of estimated clusters representation.} (a) Survival results and estimated hazard ratios over LOOCV (b-c). For Kaplan-Meier estimators, we choose a subset of curves that do not overlap too much for better visualization.}
    \label{fig:an_k16_clusters}
\end{figure}

\subsubsection{Clustered Embedding Space.}
%The learning of the feature space is performed in an fully unsupervised way and does not include any prior knowledge on tissue similarities. The validate the our model we asked pathologist to analyze and valuate the consistency of the estimated clusters. 

We fit SPKM with $K=8$ and $K=16$. The sampled tiles for each cluster are presented in Fig.~\ref{fig:an_k16_clusters}. Clusters demonstrate different tumor and stroma interactions ($c_0$, $c_1$, $c_5$, $c_9$), inflammatory tissues ($c_6$), muscles and large vessels ($c_7$), collagen and small vessels ($c_8$), blood and veins ($c_{11}$) or connective tissues ($c_{12}$). Some clusters do not directly represent the type of tissue but rather the positioning information such as $c_2$, which describe the edge of the WSI.

\input{results/table_mv_score}

\subsubsection{Ablation Study and Survival Analysis Results.}
We build our survival features (Eq.~\ref{eq:h_features}) on top of the predicted clusters, and their contribution is evaluated using Eq.~\ref{eq:forward}. In Tab.~\ref{tab_mv_score}, we observe that our model outperforms previous approaches by a safe $5\%$ margin on C-Index \cite{multivariable96harrel}. The second step of the learning (DnR w/o $\mathcal{L}_{\text{Rule}}$) tends to decrease the prediction score. Such behavior is to be expected as the additional term ($\mathcal{L}_{\text{Divide}}$) will scatter the data and focus on self instance representation. When $\mathcal{L}_{\text{Rule}}$ is then introduced, the model can restructure the embedding by linking similar instances. Also, we observe an augmentation in features, $N_{\text{feat}}$, that achieve statistical relevance for prognosis as we go through our learning procedure (for $K=16$), which proves that our proposed framework can model more subtle patches interactions. We show in Fig.~\ref{fig:an_k16_clusters} the distribution of hazard ratios for all models (from LOOCV) and the Kaplan-Meier estimator \cite{nonparam58kaplanmeier} for a subset of the selected covariates. In the best case, we identify 13 features that contribute to the survival outcome of the patients. For example, the interaction between blood vessels and tumor stroma ($h^{T}_{1\rightarrow7}$) is linked to a lower survival outcome. A similar trend observed in the relation between tumor stroma and connective tissues ($h^{T}_{0\rightarrow12}$). 





==> MICCAI 2020 - Divide and Rule/results/table_he_rgb.tex <==

\begin{table*}
\caption{\label{tab_mv_score_sup} Multivariate survival analysis comparison between self-supervised when training $\text{RGB} \rightarrow \text{RGB}$ and $\text{HE} \rightarrow \text{RGB}$. We can observe that the model performs better when we impose the color conversion from the HE space.}
\centering
\begin{threeparttable}
\begin{tabular}{l l l r d{2.5} r d{2.5}}
\toprule
 &  &  & \multicolumn{2}{c}{$\mathcal{D}^{S \cap HF}\ (n=253)$ } & \multicolumn{2}{c}{$\mathcal{D}^{S}\ (n=374)$} \\
\cmidrule(lr){4-5} \cmidrule(lr){6-7}
Method & $K$ & $\text{N}_\text{feat}$ & Brier & \multicolumn{1}{c}{C-Index} & Brier& \multicolumn{1}{c}{C-Index}\\
\midrule
$\text{MSE}_{\text{RGB} \rightarrow \text{RGB}}$ & 8 & 2 & 0.2848 & 0.5272\tnote{**} & 0.2859 & 0.5110\tnote{*}  \\
$\text{MSE}_{\text{HE} \rightarrow \text{RGB}}$ & 8 & 3 & 0.2870 & 0.6070\tnote{*} & 0.2824 & 0.6040\tnote{***}  \\
\midrule
$\text{MSE}_{\text{RGB} \rightarrow \text{RGB}}$ & 16 & 0 & 0.2893 & 0.5000 & 0.2896 & 0.5000   \\
$\text{MSE}_{\text{HE} \rightarrow \text{RGB}}$ & 16 & 5 & \textbf{0}.\textbf{2819} & \textbf{0}.\textbf{6364}\tnote{*} & \textbf{0}.\textbf{2795} & \textbf{0}.\textbf{6324}\tnote{***}   \\
\bottomrule
\end{tabular}
\begin{tablenotes}

\small
\item[+]\ $p<0.1$; $^{*}\ p<0.05$; $^{**}\ p<0.01$; $^{***}\ p<0.001$ (log-rank test).
\end{tablenotes}
\end{threeparttable}
\end{table*}

==> MICCAI 2020 - Divide and Rule/results/table_hr_bern.tex <==

\begin{table*}
\caption{\label{tab_hr_bern} Hazard ratios (HRs) with confidence intervals (CIs) based on histopathological features for $n=374$ patients with adenocarcinoma (241 right censored samples). Results are given for the univariate Cox model. If entry is non-binary, we apply one-vs.-all test.}
\centering
\begin{threeparttable}
\begin{tabular}{llrr}
\toprule
Characteristics & Subcategories & HR (95\% CI) & $p$-value \\
\midrule
Gender ($n=374$) & Male ($n=220$) &  &  \\
   & Female ($n=154$) & 0.90 (0.64 - 1.28) & 0.5139 \\
\midrule
T category ($n=373$) & pT1-2 ($n=78$) &  &  \\
   & pT3-4 ($n=295$) & 1.67 (1.00 - 2.79) & 0.0479\tnote{*} \\
\midrule
N category ($n=366$) & pN0 ($n=186$) &  &  \\
   & pN1-2 ($n=180$)  & 2.65 (1.83 - 3.82) & $<$ 0.0001\tnote{*}\\
\midrule
M category ($n=374$) & pM0 ($n=326$) &  &  \\
   & pM1 ($n=48$) & 1.76 (1.11 - 2.78) & 0.0162\tnote{*} \\
\midrule
Tumor grade ($n=369$) & G1-2 ($n=324$) &  &  \\
   & G3 ($n=45$) & 1.54 (0.96 - 2.46) & 0.0716\\
\midrule
Lymphatic invasion ($n=351$) & L0 ($n=141$) &  &  \\
   & L1 ($n=210$) & 3.35 (2.14 - 5.23) & $<$ 0.0001\tnote{*}\\
\midrule
Vascular invasion ($n=352$) & V0 ($n=193$) &  &  \\
   & V1-2 ($n=159$) & 1.52 (1.07 - 2.16) & 0.0198\tnote{*} \\
\midrule
Tumor pushing ($n=276$) & $<25\%$ ($n=109$) &  &  \\
   & $\geq25\%$ ($n=167$) & 0.59 (0.40 - 0.87) & 0.0077\tnote{*}\\
\midrule
Tumor location ($n=352$) & Left ($n=164$) &  1.28 (0.90 - 1.83) & 0.1702 \\
   & Rectum ($n=58$) & 0.83 (0.50 - 1.36) & 0.4535 \\
   & Right ($n=130$) & 0.85 (0.58 - 1.24) & 0.3967 \\
\midrule
TNM stage ($n=372$) & I ($n=64$) & 0.45 (0.24 - 0.83) & 0.0109\tnote{*} \\
   & II ($n=114$) & 0.50 (0.33 - 0.75) & 0.0010\tnote{*} \\
   & III ($n=118$) & 1.57 (1.11 - 2.22) & 0.0102\tnote{*} \\
   & IV ($n=76$) & 2.03 (1.39 - 2.96)  & 0.0003\tnote{*} \\
\bottomrule
\end{tabular}
\begin{tablenotes}
  \item[*] Indicates statistical relevance ($\alpha = 0.05$).
\end{tablenotes}
\end{threeparttable}
\end{table*}

==> MICCAI 2020 - Divide and Rule/results/table_mv_score.tex <==
\begin{table*}[t!]
\caption{\label{tab_mv_score} Multivariate survival analysis for the proposed approach and baselines. $K$ and $\text{N}_\text{feat}$ denote the number of clusters and the number of features that achieve statistical relevance when performing forward selection ($p < 0.05$). $n$ denotes the number of patient in each set. Brier and Concordance Index are indicators of the performance.}
\centering
\begin{threeparttable}
\begin{tabular}{l l l r d{2.5} r d{2.5}}
\toprule
 &  &  & \multicolumn{2}{c}{$\mathcal{D}^{S \cap HF}\ (n=253)$ } & \multicolumn{2}{c}{$\mathcal{D}^{S}\ (n=374)$} \\
\cmidrule(lr){4-5} \cmidrule(lr){6-7}
Method & $K$ & $\text{N}_\text{feat}$ & Brier \cite{forecast50briern} & \multicolumn{1}{c}{C-Index \cite{multivariable96harrel}} & Brier& \multicolumn{1}{c}{C-Index}\\
\midrule
Histo. features (HFs) &  & 8 & 0.2896 & 0.6076\tnote{***} & - & $-$  \\
\midrule
DCS & 8 & 3 & 0.2840 & 0.5398\tnote{+} & 0.2848 & 0.5562\tnote{**}   \\
DCA${}^\dagger$ \cite{muhammad2019unsupervised} & 8 & 2 & 0.2887 & 0.5452\tnote{**} & 0.2850 & 0.5555\tnote{***}  \\
DEC${}^\dagger$ \cite{xie2016unsupervised} & 8 & 4 & 0.2884 & 0.6089\tnote{**} & 0.2830 & 0.5765\tnote{**} \\
DnR w/o $\mathcal{L}_{\text{Divide}}$, $\mathcal{L}_{\text{Rule}}$ & 8 & 3 & 0.2870 & 0.6070\tnote{*} & 0.2824 & 0.6040\tnote{***}  \\
DnR w/o $\mathcal{L}_{\text{Rule}}$ & 8 & 3 & 0.2828 & 0.5951\tnote{**} & 0.2840 & 0.5919\tnote{***} \\
DnR (ours) & 8 & 4 & 0.2854 & 0.6107\tnote{*} & 0.2832 & 0.6243\tnote{***} \\
\midrule
DCS & 16 & 9 & 0.2934 & 0.6073 & 0.2879 & 0.6464\tnote{***}  \\
DCA${}^\dagger$ \cite{muhammad2019unsupervised} & 16 & 7 & 0.2827 & 0.6246\tnote{+} & 0.2852 & 0.6322\tnote{**}  \\
DEC${}^\dagger$ \cite{xie2016unsupervised} & 16 & 7 & \textbf{0}.\textbf{2758} & 0.6410\tnote{**} & 0.2763 & 0.6426\tnote{***}  \\
DnR w/o $\mathcal{L}_{\text{Divide}}$, $\mathcal{L}_{\text{Rule}}$ & 16 & 5 & 0.2819 & 0.6364\tnote{*} & 0.2795 & 0.6324\tnote{***}  \\
DnR w/o $\mathcal{L}_{\text{Rule}}$ & 16 & 10 & 0.3006 & 0.6207\tnote{+} & 0.2934 & 0.6468\tnote{***} \\
DnR (ours) & 16 & 13 & 0.2849 & \textbf{0}.\textbf{6736}\tnote{**} & \textbf{0}.\textbf{2725} & \textbf{0}.\textbf{6943}\tnote{***} \\
\bottomrule
\end{tabular}
\begin{tablenotes}

\small
\item[$\dagger$]\ Autoencoder is replaced with the self-supervised objective function.
\item[+]\ $p<0.1$; $^{*}\ p<0.05$; $^{**}\ p<0.01$; $^{***}\ p<0.001$ (log-rank test).
\end{tablenotes}
\end{threeparttable}
\end{table*}

